Rethinking Image Super-Resolution from Training Data Perspectives

In this work, we investigate the understudied effect of the training data used for image super-resolution (SR). Most commonly, novel SR methods are developed and benchmarked on common training datasets such as DIV2K and DF2K. However, we investigate and rethink the training data from the perspectives of diversity and quality, {thereby addressing the question of ``How important is SR training for SR models?''}. To this end, we propose an automated image evaluation pipeline. With this, we stratify existing high-resolution image datasets and larger-scale image datasets such as ImageNet and PASS to compare their performances. We find that datasets with (i) low compression artifacts, (ii) high within-image diversity as judged by the number of different objects, and (iii) a large number of images from ImageNet or PASS all positively affect SR performance. We hope that the proposed simple-yet-effective dataset curation pipeline will inform the construction of SR datasets in the future and yield overall better models.

==> fig/fig_diverseg__.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/SAM_ver4.pdf}
    \caption{We filtered the dataset by the number of segments. Using a segmentation model, objects in an image are divided into segments. Then, the dataset is filtered by thresholding based on the number of objects in each image.}
    \label{fig:SAM}
\end{figure*}

==> fig/fig_flow.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/fig_intro_framework.pdf}
    \caption{Our proposed SR dataset construction scheme. First, we visualize the distribution of the intensity of JPEG compression per image in the dataset. If a large percentage of images in the dataset have high compression noise, we conclude that the dataset is not adequate for SR dataset. Next, we calculate the number of segments for each image using SAM and filter the images based on this number. Filtering by the number of segments can improve performance while reducing the number of images. }
    \label{fig:flow}
    % \vspace{40pt}
\end{figure*}

==> fig/fig_violin_plot.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/violin_comp.pdf}
    \caption{Violin plots of blockiness measure of different datasets. The graph on the left plots DF2K and a subset created by JPEG compression of DF2K, while the graph on the right plots ImageNet, PASS, and Places365. The figure shows the distribution of ImageNet and PASS are similar to that of DF2K. On the other hand, Places365 is smilar to DF2K JPEG-compressed by JPEG quality 75. \ya{it's hard to see, maybe limit y-axis to 0-150} \ya{is this places365 256-resized? I think they have multiple versions}}
    \label{fig:violin_comp}
    % \vspace{20pt}
\end{figure*}

==> latexmkrc <==
$latex = 'platex';
$bibtex = 'pbibtex';
$dvipdf = 'dvipdfmx %O -o %D %S';
$makeindex = 'mendex %O -o %D %S';


add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
 if (!($root_filename eq $_[0]))
 {
  system( "latexmk -cd -pdf \"$_[0]\"" );
 }
}

==> sec/experimental_settings.tex <==

%=========================================================
%EXPERIMENTAL SETTINGS
%=========================================================
\section{Experimental Settings}
\label{sec:method}
Section~\ref{sec:explain_dataset} introduces our experimental strategy. 
Section~\ref{sec:method} indicates our proposed methods.
Section~\ref{sec:imp_details} details the implementation adopted during training.
% 本章では, 

\subsection{Experimental strategy for the training dataset}
\label{sec:explain_dataset}
Our experimental strategy consists of three parts: (i) analysis of the effectiveness of training JPEG-compressed images, (ii) benchmarking with a training dataset for SR task, and (iii) data filtering for the SR task. The details of (i), (ii), and (iii) are described below. 

%=======How do JPEG-compressed images affect SR performance?==========================
\subsubsection{How do JPEG-compressed images affect SR training? (See Section~\ref{sec:jpeg_analysis})}
JPEG-compressed images are adversely deemed to affect SR training, but detailed experiments have not been conducted. Therefore, we perform JPEG-compression on subsets of DF2K and LSDIR designed with images with low-compression noise at various JPEG quality settings, train them, and compare the results. Also, using the blockiness measure, which is able to estimate the strength of JPEG-compression noise per image, we visualize the distribution of JPEG-compressed noisy images for various datasets to see if there is any correlation with the results of training each dataset. 


%=======Other task datasets vs SR datasets==========================
\subsubsection{ImageNet and PASS as the training data for SR (See Section~\ref{sec:main_result})}
Diversity is also considered important for SR training but has not been thoroughly explored. We train various types of SR models on ImageNet and PASS, which have high diversity and are not specifically created for SR, and compare the results with those of the SR dataset. ImageNet consists of 1000 classes of objects taken in various scenes. On the other hand, PASS consists of a wide variety of natural images taken in various regions, but to solve rights issues, it excludes images containing people. Although ImageNet was used for SR tasks in some past works, it is now of limited use such as pre-training~\cite{chen2021pre, li2021efficient, chen2023activating} in classic SR since the rise of DIV2K released as a standard SR dataset due to low-resolution images with JPEG-compression noise.  However, we validated that images in ImageNet and PASS do not negatively affect SR performance in Section~\ref{sec:jpeg_analysis}.
For the comprehensive analysis, we compare the performances using representative five models MSRResNet, EDSR, RCAN, SwinIR, and HAT on DF2K, LSDIR, ImageNet, and PASS as training datasets. 

%=======Number of segments as effect indicator==========================
\subsubsection{Number of segment as effect indicator (See Section~\ref{sec:object_num})}
While diversity in general refers to the diversity among images in a dataset, we believe that the performance of super-resolution (SR) can be improved by enhancing diversity within images. Therefore, we propose a segment-based filtering method that measures the diversity within an image using the number of segments calculated from the segmentation result by SAM\cite{Kirillov_2023_ICCV}. This method collects only images segmented into more than a certain number of segments.

As an ablation study, we first use ImageNet as a training dataset to validate the effectiveness of segment-based filtering. We train subsets of images filtered with more than 50, 100, and 150 segments, respectively, and determine a threshold for the number of segments that results in good SR performance. Subsequently, we randomly reduce the subsets created by segment-based filtering and compare them with subsets filtered by the number of objects detected using Detic (an object detection method) to confirm the superiority of the segment-based filtering method. It is important to note that these subsets are adjusted to have the same number of images.

After conducting these experiments, we compare the SR models used in Section~\ref{sec:main_result}) using ImageNet and PASS before and after applying segment-based filtering to validate whether different SR models can be improved. Additionally, to investigate the impact of data scaling, we compare the merged dataset of ImageNet and PASS before and after applying segment-based filtering.

%\input{fig/fig_use_b_measure}

\subsection{Method}
\label{sec:method}
Our goal is to quantify and streamline the process of considering JPEG-compression noise and diversity when constructing SR datasets. The process enabling this is illustrated in Figure \ref{fig:flow}. First, we analyze the JPEG compression noise of datasets using the blockiness measure to determine the suitability of the target images as SR training data. Next, we apply segment-based filtering to enhance the individual diversity of the images in the dataset. These processes ensure that only images suitable for SR are extracted.
\subsubsection{Analysis of JPEG-compression noise per image}
Frist, we compute the intensity of an image using blockiness measure for all images and analyze the distribution of JPEG-compression noise in the dataset. Figure \ref{fig:use_b_measure} shows comparison of JPEG-compressed images with different values of JPEG quality. We confirmed blockiness measure is able to estimate intensity of JPEG-compression noise.
Then, we filter by the median of the calculated blockiness measure and determine that the dataset is not suitable for SR training if it is above the threshold value. 

%\input{fig/fig_diverseg}

\subsubsection{Segment-based filtering method}
As shown in Figure~\ref{fig:SAM}, we filter datasets by the number of segments per an image. We adopt SAM as our segmentation model. While typical segmentation models perform semantic region segmentation based on class labels, SAM trains labels that do not impose semantic constraints, allowing for finer region segmentation. This enables the counting of patterns in a wide variety of objects.



\subsection{Implementation details}
\label{sec:imp_details}
\noindent\textbf{Network Architecture} Primarily, we use HAT~\cite{chen2023activating}, which has a high-performance Transformer architecture, as our SR model. However, for some experiments, we also use MSRResNet~\cite{wang2018esrgan}, EDSR~\cite{lim2017enhanced}, RCAN~\cite{zhang2018image}, and SwinIR~\cite{liang2021swinir}. It's worth noting that MSRResNet, EDSR and RCAN have CNN architectures, while SwinIR has a Transformer architecture.

\noindent\textbf{Training Setup} In section~\ref{sec:main_result}, we use the following models; MSRResNet, EDSR, RCAN, SwinIR, and HAT. In accordance with the original paper, the training setup for these models was as follows. The learning rates of all models are initialized as 0.0002. MSRResNet is trained for 1,000K iterations and the learning rate is halved at 250K. EDSR and RCAN are trained for 300K iterations and the learning rate is halved at 200K. SwinIR is trained for 500K iterations and the learning rate is halved at \{250K, 400K, 450K, 475K\}. HAT is trained for 800K iterations and the learning rate is halved at \{300K, 500K, 650K, 700K, 750K\} In addition, we use 32$\times$32, 48$\times$48 and 64$\times$64 LR patches in MSRResNet, EDSR and RCAN, SwinIR and HAT respectively. In MSRResNet, EDSR and RCAN, the mini-batch size are set to 16 and in SwinIR and HAT, set to 32 sequentially. As for EDSR, we use a pre-trained scale $\times$2 model. Throughout all the experiments, we use images with a resolution higher than 256$\times$256 pixels in ImageNet and PASS. The HR-LR image pairs are made by the bicubic method of the MATLAB function. Data augmentation is applied to the training dataset, involving random rotations of 90, 180, and 270 degrees, as well as horizontal flipping. 

\noindent\textbf{Filtering Method}  In section~\ref{sec:object_num}, we use SAM and Detic as couning segments and objects. We chose the model type ViT-H for SAM and Swin Transformer for Detic.

\noindent\textbf{Evaluation.} We use five standard benchmark datasets: Set5~\cite{bevilacqua2012low}, Set14~\cite{zeyde2012single}, Urban100~\cite{huang2015single}, B100~\cite{martin2001database}, Manga109~\cite{matsui2017sketch}. PSNR and SSIM are used as evaluation metrics.
The outcomes are assessed by PSNR and SSIM metrics on the Y channel (representing luminance) within the transformed YCbCr color space. 



%=========================================================
%EXPERIMENTAL RESULTS
%=========================================================

\section{Experimental Results}
\label{sec:result_discuss}
We conducted experiments on the SR task from the perspective of datasets.  In Section~\ref{sec:jpeg_analysis}, we analyze how training on JPEG-compressed images in SR performance. In Section~\ref{sec:main_result}, we conducted a comprehensive comparison of the results of five representative SR models, each trained on one of the four different training datasets, across five benchmark datasets. In Section~\ref{sec:object_num}, we assessed the effectiveness of filtering by the number of segments. 

%\input{fig/fig_jpeg_lr_process}



%=======How do JPEG-compressed images affect SR performance?==========================
\subsection{JPEG-compression images as SR training data}
\label{sec:jpeg_analysis}
Table~\ref{tab:jpeg_results} shows both DF2K and LSDIR show decreased performance as JPEG quality decreases. Furthermore, as shown in Figure~\ref{fig:jpeg_lr_process}, it is observed that when JPEG quality is set to 50 and 75, the PSNR decreases during training. In addition, Figure~\ref{fig:jpeg_eval} compared the results of training on DF2K compressed with various JPEG quality values. As a result, it was found that when JPEG quality was set to 50 and 75, where the PSNR decreased during training, artifacts appeared in the inference results. On the other hand, no such artifacts were observed when JPEG quality was set to 85 and 95. From these observations, we can conclude that reaching a certain compression level for the images in a dataset has a significant impact on SR performance.\\
As shown in Figure~\ref{fig:violin_comp}, the blockiness measure increases as the JPEG quality of the DF2K is lowered when the DF2K is JPEG-compressed. We also observe that the distribution of DF2K compressed with JPEG quality set to 75 and the distribution of Places365 in Figure~\ref{fig:violin_comp} are similar. In Figure~\ref{fig:lr_process_datasets}, Places365 shows the same phenomenon as DF2K compressed with JPEG quality set to 75, where the PSNR deteriorates during the training process. This indicates that a dataset consisting of images with a certain intensity of JPEG compression noise is unsuitable for SR dataset. 

%\input{tab/tab_jpeg_comparison}
%\input{fig/fig_violin_plot}
\input{fig/fig_dataset_lr_process}


%=======Other task datasets vs SR datasets==========================
%This section is under revision.
\subsection{Comparison of the performance among SR datasets, ImageNet, and PASS}
\label{sec:main_result}
As shown in Table~\ref{tab:main_quantitative}, the performance achieved when training on ImageNet and PASS is superior to that obtained when training on DF2K, especially when compared to Urban100 and Manga109. When evaluated on Urban100, MSRResNet, EDSR, RCAN, SwinIR, and HAT trained on ImageNet exhibited higher PSNR values by 0.06 to 0.48 dB, respectively, compared to those trained on DF2K. Similarly, these models trained on PASS showed higher differences of 0.05 to 0.55 dB, respectively. While these models trained on ImageNet showed slightly inferior performance compared to those trained on LSDIR, models trained on PASS achieved comparable performance.
When evaluated on Manga109, models trained on ImageNet showed higher PSNR values (XXX to XXX dB and XXX to XXX dB) compared to those trained on DF2K and LSDIR. In the same way, models trained PASS, except for EDVR trained on LSDIR, demonstrated higher PSNR values (XXX to XXX dB and XXX to XXX dB) compared to DF2K and LSDIR. 

Additionally, Figure~\ref{fig:main_qualitative} shows visual comparisons of the aforementioned models. For ``image\_011" in Urban100, we observe that models trained on DF2K cannot recover the lattice content. On the other hand, models trained on ImageNet and PASS, respectively, successfully recovers the above content as well as trained on LSDIR. We can also observe enhancement of the character region on ``YumeiroCokking", ``ShimatteIkouze\_vol26", and ``PlayerHaNemurenai" in Manga109. The models trained on ImageNet or PASS exhibit noticeable improvement in the character region compared to those trained on DF2K or LSDIR.

From the above comprehensive verification, it can be seen that SR datasets, which is designed for SR task, are not necessarily essential for maintaining performance, and ImageNet and PASS, which is not designed for SR task, can achieve comparable performance. 
In terms of resolution, there were no obvious shortcomings in the models trained on ImageNet or PASS. These results suggest that there are other factors that lead to improved performance apart from high-resolution images with low-compression noise.


%=======Number of segments as effect indicator==========================
\subsection{Number of segment as effect indicator}
\label{sec:object_num}

%\input{tab/tab_filters}
As shown in Table~\ref{tab:filters}, segment-based and object-based filtering methods show higher PSNR and SSIM compared to random reduction. Furthermore, segment-based filtering outperforms object-based filtering, especially for Urban100. These results indicate that images with more patterns are effective for SR training, and finer granularity leads to better performance.

Additionally, as shown in Table~\ref{tab:filters_size}, despite containing only 22.5\% of the original number of images, training on all images resulted in a 0.1dB higher PSNR for Urban100 and nearly equivalent performance for Manga109. This suggests that segment-based filtering is effective in selecting images that contribute to performance improvement.


Furthermore,Table~\ref{tab:sota} compared the performance improvement by data scaling using the threshold of 100 segments or more, which showed the best performance in the above experiments. As a result, it was found that a subset consisting of 526K images filtered with 100 segments or more outperformed a dataset consisting of 2.49M images, including ImageNet and PASS merged. Specifically, models trained on ImageNet showed a higher performance trend on Manga109, and models trained on PASS showed a higher performance trend on Urban100, but the subset mentioned above could learn both characteristics. On the other hand, such effects were not obtained by simply merging datasets. From this, it can be understood that filtering by the number of segments removes images that are not suitable for SR.

In the realm of SR tasks, the characteristics of data are often examined through the lens of high and low-frequency components. Nevertheless, when performing frequency-based filtering, there exists a substantial risk of introducing bias to the target object, and this bias may not be assured when contemplating data diversity. In contrast, our proposed filtering method based on the number of segments enables the identification of essential data diversity for SR from the perspective of object diversity.






\subsection{Discussion and Limitations}
\noindent\textbf{Needs for SR datasets.} In Section~\ref{sec:main_result}, we quantitatively and qualitatively verified that even general datasets like ImageNet and PASS are valuable as training datasets for SR tasks when compared to carefully constructed SR datasets (e.g., DF2K and LSDIR). Conventionally, dataset construction has been performed by annotators, who cross-check under specific conditions of resolution and compression ratio. However, this extensive cross-checking may not always be necessary. Moving forward, dataset construction is anticipated to shift towards automated creation, leveraging web crawling like image recognition field, which previously were time-consuming processes.
 
\noindent\textbf{The effect of data filtering by segment counting.} In this paper, we propose a new data filtering method for SR, serving as an alternative to traditional human cross-checking. As detailed in Section \ref{sec:object_num}, our findings demonstrate that performance enhancement is achieved by segment-based filtering. Specifically, within the Urban100 dataset, a correlation was observed between the performance metrics and the average frequency in the training dataset. This correlation may stem from the high-textured components in Urban100, such as window grids on buildings, suggesting that training with datasets having higher frequencies can be beneficial. Given these findings, it is critical to carefully consider the characteristics of the datasets under evaluation during the design phase.


\noindent\textbf{Filtering by blockiness measure.}
We trained on ImageNet using the results from filtering with various thresholds of blockiness measure and compared the results. As shown in the Table~\ref{tab:filters_b}, the filtering did not affect PSNR of Urban100, but a decrease in PSNR was observed for Manga109. From these results, it is possible that JPEG-compressed images not only do not have a negative impact on their own but also contribute to performance improvement.

\noindent\textbf{High resolution images for SR.}


\noindent\textbf{Limitations.} While our experiments have demonstrated the utility of general datasets like ImageNet and PASS in SR, comparable to SR datasets, it is important to acknowledge that there may be unknown drawbacks not observable through evaluations based on PSNR, SSIM, or qualitative visual assessments. Further analysis is required to clearly delineate what aspects are beneficial or detrimental in SR datasets.  


==> sec/introduction.tex <==
\section{Introduction}
\label{sec:intro}
Image super-resolution (SR), which reconstructs a high-resolution image from a low-resolution image, has been treated as one of the fundamental vision task in computer vision.  Deep neural networks have led to significant advances in SR, focusing primarily on improvements for the architecture of models. A variety of models based on convolutional neural networks (CNN) have been proposed for SR~\cite{dong2014learning, kim2016accurate, dong2016accelerating, shi2016real, ledig2017photo, tai2017image, lim2017enhanced, zhang2018residual, zhang2018image}. Recent innovations have given rise to transformer-based models~\cite{chen2021pre, li2021efficient, liang2021swinir, chen2023activating}, setting new benchmarks and consistently pushing the performance boundaries.

\input{fig/fig_overview}



With the improvement in model performance, the importance of datasets has also increased. While the focus of performance enhancement has traditionally been on the design of the model architecture also as mentioned in ~\cite{Li_2023_CVPR}, it has been confirmed that training on large-scale datasets significantly contributes to performance improvement. Regarding SR datasets, DF2K, a merged dataset of DIV2K~\cite{agustsson2017ntire} and Flickr2K~\cite{timofte2017ntire}, is commonly used as a training dataset consisting of 3,450 images. More recently, LSDIR~\cite{Li_2023_CVPR}, which contains 84,991 images, ten times more than DF2K, has been proposed.

SR datasets are constructed through web crawling, following the same approach as in other tasks.
Nevertheless, in contrast to other tasks, it has been deemed necessary to consider the following elements.
\begin{itemize}
  \item JPEG-compression noise; images with high-compressed noise are purported to adversely affect the SR training results~\cite{Li_2023_CVPR,yang2023hq}.
  \item Diversity; images with abundant texture and color information contribute to SR performance~\cite{chen2021pre}.
  \item Frequency components; XXX~\cite{li2023feature}
  \item Resolution; low-resolution images are considered unsuitable for training data~\cite{Li_2023_CVPR,yang2023hq}.
\end{itemize}  

However, the construction of SR datasets with the above two factors is approached qualitatively. Therefore, constructing datasets requires extensive manual labor, which makes building SR datasets challenging. Additionally, experiments regarding these elements have not been conducted. it is now imperative to reconsider SR datasets. Thus, we investigate the extent to which JPEG-compressed images and diversity affect SR performance. As the results, we obtain the following findings (i) (ii) (iii).

\input{fig/fig_flow}

\noindent \textbf{(i) Percentage of JPEG-compressed images is important}:  At the beginning of the investiation, we investigate the effectiveness of using JPEG-compressed images as SR training data. First, we JPEG-compress DF2K and LSDIR, which consist of low-compression images, into several subsets with varying JPEG quality and train SR models on them. Then, it was found that the lower the JPEG quality value, the lower the performance. Additionally, for the subset with low JPEG quality, we observed that performance began to degrade during the training process. Furthermore, we use blockiness measure~\cite{bhardwaj2018jpeg}, which is able to calculate the degree of degradation caused by JPEG compression, and visualize the distribution of JPEG compression noise of the images in different datasets. The results showed that when the percentage of images with a high degree of JPEG compression reaches a certain level, artifacts are generated in the inference results, leading to performance degradation.

\noindent \textbf{(ii) Diversity is a key factor for SR}: To investigate the extent to which diversity contributes to SR performance, we compare the results of different representative models trained on SR datasets (DF2K and LSDIR), ImageNet and PASS~\cite{asano21pass}, datasets with excellent diversity and devoid of the negative effects of JPEG-compression noise, within an experimental framework. As the result, ImageNet and PASS are comparable to SR datasets on Urban100 and superior to them on Manga109. The above results suggest diversity may be more important for SR than previously thought.

\noindent \textbf{(iii) Segment-based filtering improves SR performance}: The diversity mentioned in (ii) refers to the diversity among images, but we wonder if improving the diversity within images would also improve the performance of SR. Therefore, assuming that the number of segments can measure diversity within an image, we propose a segment-based filtering method that collects only images segmented by over a certain number of segments. Frist, we train the SR model on ImageNet and PASS filtered by segment-based filtering. Here, we observe that the results of ImageNet and PASS filtered with thresholds of 100 or more, outperformed the result of the entire ImageNet. These subsets, comprising 20\％ of the entire ImageNet, achieve higher performance than the overall ImageNet despite the smaller number of images. Furthermore, merged subsets of ImageNet and PASS filtered by more than 100 segments lead to better SR performance than merged ImageNet and PASS.

The above results indicates that our findings improve the construction of SR datasets in a data-efficient manner. It is expected to alleviate the problems in the construction of conventional SR datasets and serve as a guideline for constructing future SR datasets. 


==> tab/tab_comparison_finetuning.tex <==
\begin{table}[h]
\center
\begin{center}
\vspace{-0.3cm}
\scalebox{0.60}{
\begin{tabular}{c|cc|cc|cc|cc}
\toprule
Our experiments& \multicolumn{2}{c|}{Set5}& \multicolumn{2}{c|}{Set14}&  \multicolumn{2}{c|}{Urban100} & \multicolumn{2}{c}{Manga109} \\
 (SR$\times$4)   &            PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\
\midrule
ImageNet                 &33.08  &0.9071  &29.40  &0.7999   &28.41  &0.8457 &32.88  &0.9323    \\
ImageNet$\to$DF2K        &\textbf{33.18}  &\textbf{0.9074}  &29.38  &0.7998  &28.40  &0.8453  &32.89 &0.9322    \\
DiverSeg-I (Ours)        &33.15  &0.9071  &\textbf{29.46}  &\textbf{0.8004}  &\textbf{28.51}  &\textbf{0.8477}  & \textbf{32.90} & \textbf{0.9325}\\

\bottomrule
\end{tabular}
}
\vspace{-0.3cm}
\end{center}
\end{table}

==> tab/tab_discussion_distortion.tex <==
\begin{table}[h]
\center
\centering
\caption{Comparison of the robustness of our filtering method against various image distortions.
}
\begin{center}
\label{tab:discuss_distortion}
\scalebox{0.99}{

\begin{tabular}{c|c|c|c}
\toprule
Distortions&
Parameter & Blockiness (median) & \#Segments (average)\\
\midrule
   -      & -          &0.47   &103     \\ 
\hline
\hline
         & $s=8$  &12.21       & 98   \\
Rescaling\tablefootnote{Bicubic interpolation: downscale and upscale by a scale factor s.}  & $s=12$ &0.32       & 84  \\
          & $s=16$ & 1.34      & 73     \\ 
\hline
\hline
          & $\sigma_b=4$   &0.33       &100 \\
Blurring\tablefootnote{Gaussian blur: set the kernel size to (21, 21) and control the blur intensity with the standard deviation of the Gaussian distribution $\sigma_b$.}  & $\sigma_b=6$   &0.31       &89 \\
         & $\sigma_b=8$   &0.32        &83 \\
\hline
\hline
         & $\sigma_n=20$ &0.34      & 98 \\
Noises\tablefootnote{Color Gaussian noise: control the noise intensity with the standard deviation of the Gaussian distribution $\sigma_n$.}   & $\sigma_n=30$ &0.32       & 95 \\
        & $\sigma_n=40$ &0.32      & 91 \\
\bottomrule
\end{tabular}
}
% \vspace{-0.4cm}
\end{center}
\end{table}

==> tab/tab_fair_comparison.tex <==
\begin{table}[t]
\center
\begin{center}
% \caption{Fair quantitative comparison of DF2K and our datasets on three benchmark datasets. We adopt HAT model.
% }
% \label{tab:fair_comparison}

% \vspace{-0.4cm}
% \vspace{-0.2cm}
% \renewcommand{\arraystretch}{1.1}
% \linespread{1.3}
\centering
\caption{Fair comparison of DiverSeg and DF2K with comparable numbers of pixels.
}
\label{tab:fair_comp}
\scalebox{0.75}{
\resizebox{\linewidth}{!}{
% \setlength{\tabcolsep}{1mm}{
\begin{tabular}{l|c|cc|cc|cc}
\toprule
{Scale} & {Training Data} & 
\multicolumn{2}{c|}{Set14} &  \multicolumn{2}{c|}{Urban100} &  \multicolumn{2}{c}{Manga109}  
\\ 
& & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM
\\ 
\hline
\hline
$\times$2 & DF2K
& {34.86}
& {0.9274}
& {34.45}
& {0.9466}
& {40.26}
& {0.9809}
\\
$\times$2 & DiverSeg-I\_S 
& \textbf{35.14}
& \textbf{0.9283}
& 34.94
& 0.9498
& \textbf{40.73}
& \textbf{0.9819}
\\
$\times$2 & DiverSeg-P\_S
& 35.13
& 0.9275
& \textbf{35.07}
& \textbf{0.9502}
& 40.34
& 0.9807
\\
\hline
\hline
$\times$3 & DF2K
& {31.08}
& {0.8555}
& {30.23}
& {0.8896}
& {35.53}
& {0.9552}
\\
$\times$3 & DiverSeg-I\_S 
& 31.34
& 0.8561
& 30.59
& 0.8942
& \textbf{35.73}
& \textbf{0.9563}
\\
$\times$3 & DiverSeg-P\_S 
& \textbf{31.46}
& \textbf{0.8566}
& \textbf{30.76}
& \textbf{0.8963}
& 35.67
& 0.9559
\\
\hline
\hline
$\times$4 & DF2K
& 29.23
& 0.7973
& 27.97
& 0.8368
& 32.48
& 0.9292
\\
$\times$4 & DiverSeg-I\_S 
& 29.34
& 0.7988
& 28.15
& 0.8418
& \textbf{32.71}
& \textbf{0.9311}
\\
$\times$4 & DiverSeg-P\_S 
& \textbf{29.38}
& \textbf{0.7990}
& \textbf{28.27}
& \textbf{0.8447}
& 32.68
& 0.9310
\\
\bottomrule
\end{tabular}
}}
% \vspace{-0.4cm}
\vspace{-0.2cm}
\end{center}
\end{table}

==> tab/tab_sota_x2.tex <==
\begin{table}[t]
\center
\begin{center}
\caption{Quantitative comparison with state-of-the-art methods on five benchmark datasets. We applied our dataset to two Transformer-based models.
Checkmarks for HR, LR indicate the use of high-resolution and low-resolution datasets, respectively.
}
\label{tab:sota}
\tablevspacemid
%\vspace{-0.5cm}
% \renewcommand{\arraystretch}{1.1}
% \linespread{1.3}
\resizebox{\linewidth}{!}{
% \setlength{\tabcolsep}{1mm}{
\begin{tabular}{l|c|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Training Data} & \multirow{2}{*}{HR} & \multirow{2}{*}{LR} &
\multicolumn{2}{c|}{Set5} &  \multicolumn{2}{c|}{Set14} &  \multicolumn{2}{c|}{BSD100} &  \multicolumn{2}{c|}{Urban100} &  \multicolumn{2}{c}{Manga109}  
\\ 
& & & & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM 
\\ 
\midrule
%EDSR & DIV2K & $\checkmark$ & %& 32.46 & 0.8968 & 28.80 & 0.7876 & 27.71 & 0.7420 & 26.64 & 0.8033 & 31.02 & 0.9148 \\
%EDSR & DiverSeg-I (Ours) & & $\checkmark$ % & \textbf{32.71} & \textbf{0.9017}  & \textbf{28.98} & \textbf{0.7913}  & \textbf{27.85} & \textbf{0.7453}  & \textbf{27.10} & \textbf{0.8142}  & \textbf{31.72} & \textbf{0.9216} \\
%\midrule
%RCAN & DIV2K & $\checkmark$ & % & 32.63 & 0.9002 & 28.87 & 0.7889 & 27.77 & 0.7436 & 26.82 & 0.8087 & 31.22 & 0.9173 \\
SAN~\cite{dai2019second} & DIV2K & $\checkmark$ & %
& {38.31}
& {0.9620}
& {34.07}
& {0.9213}
& {32.42}
& {0.9028}
& {33.10}
& {0.9370}
& {39.32}
& {0.9792}
\\
IGNN~\cite{zhou2020cross} & DIV2K & $\checkmark$ & %
& {38.24}
& {0.9613}
& {34.07}
& {0.9217}
& {32.41}
& {0.9025}
& {33.23}
& {0.9383}
& {39.35}
& {0.9786}
\\
HAN~\cite{niu2020single} & DIV2K & $\checkmark$ & %
& {38.27}
& {0.9614}
& {34.16}
& {0.9217}
& {32.41}
& {0.9027}
& {33.35}
& {0.9385}
& {39.46}
& {0.9785} 
\\
NLSN~\cite{mei2021image} & DIV2K & $\checkmark$ & %
& 38.34 
& 0.9618 
& 34.08 
& 0.9231
& 32.43 
& 0.9027 
& 33.42
& 0.9394
& 39.59
& 0.9789
\\
RCAN-it~\cite{lin2022revisiting} & DF2K & $\checkmark$ & %
& 38.37
& 0.9620
& 34.49
& 0.9250
& 32.48
& 0.9034
& 33.62
& 0.9410
& 39.88
& 0.9799
\\
EDT~\cite{li2021efficient} & DF2K & $\checkmark$ & %
& 38.45
& 0.9624
& 34.57
& 0.9258
& 32.52
& 0.9041
& 33.80
& 0.9425
& 39.93
& 0.9800
\\
HAT-S~\cite{chen2023activating} & DF2K & $\checkmark$ & %
& {38.58}
& {0.9628}
& {34.70}
& {0.9261}
& {32.59}
& {0.9050}
& {34.31}
& {0.9459}
& {40.14}
& {0.9805}
\\
\hdashline
IPT~\cite{chen2021pre} & ImageNet & & $\checkmark$ %
& {38.37}
& {-}
& {34.43}
& {-}
& {32.48}
& {-}
& {33.76}
& {-}
& {-}
& {-}
\\
%EDT & ImageNet$\to$DF2K & $\checkmark$ & $\checkmark$ % & 33.06 & {0.9055} & 29.23 & {0.7971} & {27.99} & 0.7510 & 27.75 & 0.8317 & 32.39 & 0.9283 \\
%\midrule
%RCAN & DiverSeg-I (Ours) & & $\checkmark$ % & \textbf{32.70} & \textbf{0.9012} & \textbf{28.98} & \textbf{0.7908} & \textbf{27.81} & \textbf{0.7443} & \textbf{27.03} & \textbf{0.8116} & \textbf{31.58} & \textbf{0.9210}\\
\midrule
SwinIR~\cite{liang2021swinir} & DF2K & $\checkmark$ & %
& 38.42
& 0.9623
& 34.46
& 0.9250
& 32.53
& 0.9041
& 33.81
& 0.9427
& 39.92
& 0.9797
\\
SwinIR~\cite{liang2021swinir} & DiverSeg-I (Ours) & & $\checkmark$
& \textbf{38.50}
& \textbf{0.9628}
& \textbf{34.80}
& \textbf{0.9268}
& \textbf{32.61}
& \textbf{0.9051}
& \textbf{34.36}
& \textbf{0.9460}
& \textbf{40.38}
& \textbf{0.9812}
\\
\midrule
HAT~\cite{chen2023activating} & DF2K & $\checkmark$ & %
& {38.63}
& {0.9630}
& {34.86}
& {0.9274}
& {32.62}
& {0.9053}
& {34.45}
& {0.9466}
& {40.26}
& {0.9809}
\\
HAT~\cite{chen2023activating} & ImageNet$\to$DF2K & $\checkmark$ & $\checkmark$ %
& {38.73}
& \textbf{0.9637}
& {35.13}
& {0.9282}
& {32.69}
& {0.9060}
& {34.81}
& {0.9489}
& {40.71}
& {0.9819}
\\
HAT~\cite{chen2023activating} & DiverSeg-I (Ours) & & $\checkmark$ %
& \textbf{38.75}
& 0.9636
& \textbf{35.18}
& \textbf{0.9284}
& \textbf{32.74}
& \textbf{0.9065}
& 35.06
& 0.9502
& \textbf{40.78}
& \textbf{0.9821}
\\
HAT~\cite{chen2023activating} & DiverSeg-IP (Ours) & & $\checkmark$ %
& 38.72
& 0.9634
& \textbf{35.18}
& 0.9283
& 32.73
& 0.9064
& \textbf{35.10}
& \textbf{0.9504}
& 40.70
& 0.9819

\\

\bottomrule
\end{tabular}
}
%\vspace{-0.5cm}
\end{center}
\end{table}

==> tab/tab_sota_x2x3.tex <==
\begin{table}[h]
\center
\begin{center}
\caption{Quantitative comparison with state-of-the-art methods on five benchmark datasets. We applied our dataset to two Transformer-based models.
Checkmarks for HR, LR indicate the use of high-resolution and low-resolution datasets, respectively.
}
\label{tab:sota_x2x3}
\tablevspacemid
%\vspace{-0.5cm}
% \renewcommand{\arraystretch}{1.1}
% \linespread{1.3}
\scalebox{1.0}{
\resizebox{\linewidth}{!}{
% \setlength{\tabcolsep}{1mm}{
\begin{tabular}{l|c|c|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method}& \multirow{2}{*}{Scale} & \multirow{2}{*}{Training Data} & \multirow{2}{*}{HR} & \multirow{2}{*}{LR} &
\multicolumn{2}{c|}{Set5} &  \multicolumn{2}{c|}{Set14} &  \multicolumn{2}{c|}{BSD100} &  \multicolumn{2}{c|}{Urban100} &  \multicolumn{2}{c}{Manga109}  
\\ 
& & & & & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM 
\\ 
\hline
\hline
%EDSR & DIV2K & $\checkmark$ & %& 32.46 & 0.8968 & 28.80 & 0.7876 & 27.71 & 0.7420 & 26.64 & 0.8033 & 31.02 & 0.9148 \\
%EDSR & DiverSeg-I (Ours) & & $\checkmark$ % & \textbf{32.71} & \textbf{0.9017}  & \textbf{28.98} & \textbf{0.7913}  & \textbf{27.85} & \textbf{0.7453}  & \textbf{27.10} & \textbf{0.8142}  & \textbf{31.72} & \textbf{0.9216} \\
%\midrule
%RCAN & DIV2K & $\checkmark$ & % & 32.63 & 0.9002 & 28.87 & 0.7889 & 27.77 & 0.7436 & 26.82 & 0.8087 & 31.22 & 0.9173 \\
SAN~\cite{dai2019second} & $\times$2 & DIV2K & $\checkmark$ & %
& {38.31}
& {0.9620}
& {34.07}
& {0.9213}
& {32.42}
& {0.9028}
& {33.10}
& {0.9370}
& {39.32}
& {0.9792}
\\
IGNN~\cite{zhou2020cross} & $\times$2 & DIV2K & $\checkmark$ & %
& {38.24}
& {0.9613}
& {34.07}
& {0.9217}
& {32.41}
& {0.9025}
& {33.23}
& {0.9383}
& {39.35}
& {0.9786}
\\
HAN~\cite{niu2020single} & $\times$2 & DIV2K & $\checkmark$ & %
& {38.27}
& {0.9614}
& {34.16}
& {0.9217}
& {32.41}
& {0.9027}
& {33.35}
& {0.9385}
& {39.46}
& {0.9785} 
\\
NLSN~\cite{mei2021image} & $\times$2 & DIV2K & $\checkmark$ & %
& 38.34 
& 0.9618 
& 34.08 
& 0.9231
& 32.43 
& 0.9027 
& 33.42
& 0.9394
& 39.59
& 0.9789
\\
RCAN-it~\cite{lin2022revisiting} & $\times$2 & DF2K & $\checkmark$ & %
& 38.37
& 0.9620
& 34.49
& 0.9250
& 32.48
& 0.9034
& 33.62
& 0.9410
& 39.88
& 0.9799
\\
EDT~\cite{li2021efficient} & $\times$2 & DF2K & $\checkmark$ & %
& 38.45
& 0.9624
& 34.57
& 0.9258
& 32.52
& 0.9041
& 33.80
& 0.9425
& 39.93
& 0.9800
\\
HAT-S~\cite{chen2023activating} & $\times$2 & DF2K & $\checkmark$ & %
& {38.58}
& {0.9628}
& {34.70}
& {0.9261}
& {32.59}
& {0.9050}
& {34.31}
& {0.9459}
& {40.14}
& {0.9805}
\\
\hdashline
IPT~\cite{chen2021pre} & $\times$2 & ImageNet & & $\checkmark$ %
& {38.37}
& {-}
& {34.43}
& {-}
& {32.48}
& {-}
& {33.76}
& {-}
& {-}
& {-}
\\
%EDT & ImageNet$\to$DF2K & $\checkmark$ & $\checkmark$ % & 33.06 & {0.9055} & 29.23 & {0.7971} & {27.99} & 0.7510 & 27.75 & 0.8317 & 32.39 & 0.9283 \\
%\midrule
%RCAN & DiverSeg-I (Ours) & & $\checkmark$ % & \textbf{32.70} & \textbf{0.9012} & \textbf{28.98} & \textbf{0.7908} & \textbf{27.81} & \textbf{0.7443} & \textbf{27.03} & \textbf{0.8116} & \textbf{31.58} & \textbf{0.9210}\\
\midrule
SwinIR~\cite{liang2021swinir} & $\times$2 & DF2K & $\checkmark$ & %
& 38.42
& 0.9623
& 34.46
& 0.9250
& 32.53
& 0.9041
& 33.81
& 0.9427
& 39.92
& 0.9797
\\
SwinIR~\cite{liang2021swinir} & $\times$2 & DiverSeg-I (Ours) & & $\checkmark$
& \textbf{38.50}
& \textbf{0.9628}
& \textbf{34.78}
& \textbf{0.9268}
& \textbf{32.63}
& \textbf{0.9052}
& \textbf{34.35}
& \textbf{0.9460}
& \textbf{40.40}
& \textbf{0.9812}
\\
\midrule
HAT~\cite{chen2023activating} & $\times$2 & DF2K & $\checkmark$ & %
& {38.63}
& {0.9630}
& {34.86}
& {0.9274}
& {32.62}
& {0.9053}
& {34.45}
& {0.9466}
& {40.26}
& {0.9809}
\\
HAT~\cite{chen2023activating} & $\times$2 & ImageNet$\to$DF2K & $\checkmark$ & $\checkmark$ %
& {38.73}
& \textbf{0.9637}
& {35.13}
& {0.9282}
& {32.69}
& {0.9060}
& {34.81}
& {0.9489}
& {40.71}
& {0.9819}
\\
HAT~\cite{chen2023activating} & $\times$2 & DiverSeg-I (Ours) & & $\checkmark$ %
& \textbf{38.75}
& 0.9636
& \textbf{35.18}
& \textbf{0.9284}
& \textbf{32.74}
& \textbf{0.9065}
& 35.06
& 0.9502
& \textbf{40.78}
& \textbf{0.9821}
\\
HAT~\cite{chen2023activating} & $\times$2 & DiverSeg-IP (Ours) & & $\checkmark$ %
& 38.72
& 0.9634
& \textbf{35.18}
& 0.9283
& 32.73
& 0.9064
& \textbf{35.10}
& \textbf{0.9504}
& 40.70
& 0.9819
\\
\hline
\hline
SAN~\cite{dai2019second} & $\times$3 & DIV2K & $\checkmark$ & %
& {34.75}
& {0.9300}
& {30.59}
& {0.8476}
& {29.33}
& {0.8112}
& {28.93}
& {0.8671}
& {34.30}
& {0.9494}
\\
IGNN~\cite{zhou2020cross} & $\times$3 & DIV2K & $\checkmark$ & %
& {34.72}
& {0.9298}
& {30.66}
& {0.8484}
& {29.31}
& {0.8105}
& {29.03}
& {0.8696}
& {34.39}
& {0.9496}
\\
HAN~\cite{niu2020single} & $\times$3 & DIV2K & $\checkmark$ & %
& {34.75}
& {0.9299}
& {30.67}
& {0.8483}
& {29.32}
& {0.8110}
& {29.10}
& {0.8705}
& {34.48}
& {0.9500}
\\
NLSN~\cite{mei2021image} & $\times$3 & DIV2K & $\checkmark$ & %
& 34.85 
& 0.9306 
& 30.70 
& 0.8485 
& 29.34 
& 0.8117 
& {29.25}
& {0.8726}
& 34.57 
& 0.9508 
\\
RCAN-it~\cite{lin2022revisiting} & $\times$3 & DF2K & $\checkmark$ & %
& {34.86}
& {0.9308}
& {30.76}
& {0.8505}
& {29.39}
& {0.8125}
& {29.38}
& {0.8755}
& {34.92}
& {0.9520}
\\
EDT~\cite{li2021efficient} & $\times$3 & DF2K & $\checkmark$ & %
& 34.97
& 0.9316
& 30.89
& 0.8527
& 29.44
& 0.8142
& 29.72
& 0.8814
& 35.13
& 0.9534
\\
HAT-S~\cite{chen2023activating} & $\times$3 & DF2K & $\checkmark$ & %
& {35.01}
& {0.9325}
& {31.05}
& {0.8550}
& {29.50}
& {0.8158}
& {30.15}
& {0.8879}
& {35.40}
& {0.9547}
\\
\hdashline
IPT~\cite{chen2021pre} & $\times$3 & ImageNet & & $\checkmark$ %
& {34.81}
& {-}
& {30.85}
& {-}
& {29.38}
& {-}
& {29.49}
& {-}
& {-}
& {-}
\\
%EDT & ImageNet$\to$DF2K & $\checkmark$ & $\checkmark$ % & 33.06 & {0.9055} & 29.23 & {0.7971} & {27.99} & 0.7510 & 27.75 & 0.8317 & 32.39 & 0.9283 \\
%\midrule
%RCAN & DiverSeg-I (Ours) & & $\checkmark$ % & \textbf{32.70} & \textbf{0.9012} & \textbf{28.98} & \textbf{0.7908} & \textbf{27.81} & \textbf{0.7443} & \textbf{27.03} & \textbf{0.8116} & \textbf{31.58} & \textbf{0.9210}\\
\midrule
SwinIR~\cite{liang2021swinir} & $\times$3 & DF2K & $\checkmark$ & %
& 34.97
& 0.9318
& 30.93
& 0.8534
& 29.46
& 0.8145
& 29.75
& 0.8826
& 35.12
& 0.9537
\\
SwinIR~\cite{liang2021swinir} & $\times$3 & DiverSeg-I (Ours) &  & $\checkmark$
& \textbf{35.00}
& \textbf{0.9321}
& \textbf{31.11}
& \textbf{0.8544}
& \textbf{29.50}
& \textbf{0.8160}
& \textbf{30.11}
& \textbf{0.8868}
& \textbf{35.40}
& \textbf{0.9548}
\\
\midrule
HAT~\cite{chen2023activating} & $\times$3 & DF2K & $\checkmark$ & %
& {35.07}
& {0.9329}
& {31.08}
& {0.8555}
& {29.54}
& {0.8167}
& {30.23}
& {0.8896}
& {35.53}
& {0.9552}
\\
HAT~\cite{chen2023activating} & $\times$3 & ImageNet$\to$DF2K & $\checkmark$ & $\checkmark$ %
& \textbf{35.16}
& \textbf{0.9335}
& {31.33}
& {0.8576}
& {29.59}
& {0.8177}
& {30.70}
& {0.8949}
& \textbf{35.84}
& \textbf{0.9567}
\\
HAT~\cite{chen2023activating} & $\times$3 & DiverSeg-I (Ours) & & $\checkmark$ %
& 35.14
& 0.9334
& 31.42
& \textbf{0.8577}
& \textbf{29.60}
& 0.8187
& 30.83
& 0.8965
& 35.80
& 0.9566
\\
HAT~\cite{chen2023activating} & $\times$3  & DiverSeg-IP (Ours) & & $\checkmark$ %
& 35.10
& 0.9333
& \textbf{31.49}
& 0.8574
& \textbf{29.60}
& \textbf{0.8188}
& \textbf{30.94}
& \textbf{0.8982}
& \textbf{35.84}
& \textbf{0.9567}
\\
\bottomrule
\end{tabular}
}}
%\vspace{-0.5cm}
\end{center}
\end{table}

==> tab/tab_sota_x3.tex <==
\begin{table}[t]
\center
\begin{center}
\caption{Quantitative comparison with state-of-the-art methods on five benchmark datasets. We applied our dataset to two Transformer-based models.
Checkmarks for HR, LR indicate the use of high-resolution and low-resolution datasets, respectively.
}
\label{tab:sota}
\tablevspacemid
%\vspace{-0.5cm}
% \renewcommand{\arraystretch}{1.1}
% \linespread{1.3}
\resizebox{\linewidth}{!}{
% \setlength{\tabcolsep}{1mm}{
\begin{tabular}{l|c|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Training Data} & \multirow{2}{*}{HR} & \multirow{2}{*}{LR} &
\multicolumn{2}{c|}{Set5} &  \multicolumn{2}{c|}{Set14} &  \multicolumn{2}{c|}{BSD100} &  \multicolumn{2}{c|}{Urban100} &  \multicolumn{2}{c}{Manga109}  
\\ 
& & & & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM 
\\ 
\midrule
%EDSR & DIV2K & $\checkmark$ & %& 32.46 & 0.8968 & 28.80 & 0.7876 & 27.71 & 0.7420 & 26.64 & 0.8033 & 31.02 & 0.9148 \\
%EDSR & DiverSeg-I (Ours) & & $\checkmark$ % & \textbf{32.71} & \textbf{0.9017}  & \textbf{28.98} & \textbf{0.7913}  & \textbf{27.85} & \textbf{0.7453}  & \textbf{27.10} & \textbf{0.8142}  & \textbf{31.72} & \textbf{0.9216} \\
%\midrule
%RCAN & DIV2K & $\checkmark$ & % & 32.63 & 0.9002 & 28.87 & 0.7889 & 27.77 & 0.7436 & 26.82 & 0.8087 & 31.22 & 0.9173 \\
SAN~\cite{dai2019second} & DIV2K & $\checkmark$ & %
& {34.75}
& {0.9300}
& {30.59}
& {0.8476}
& {29.33}
& {0.8112}
& {28.93}
& {0.8671}
& {34.30}
& {0.9494}
\\
IGNN~\cite{zhou2020cross} & DIV2K & $\checkmark$ & %
& {34.72}
& {0.9298}
& {30.66}
& {0.8484}
& {29.31}
& {0.8105}
& {29.03}
& {0.8696}
& {34.39}
& {0.9496}
\\
HAN~\cite{niu2020single} & DIV2K & $\checkmark$ & %
& {34.75}
& {0.9299}
& {30.67}
& {0.8483}
& {29.32}
& {0.8110}
& {29.10}
& {0.8705}
& {34.48}
& {0.9500}
\\
NLSN~\cite{mei2021image} & DIV2K & $\checkmark$ & %
& 34.85 
& 0.9306 
& 30.70 
& 0.8485 
& 29.34 
& 0.8117 
& {29.25}
& {0.8726}
& 34.57 
& 0.9508 
\\
RCAN-it~\cite{lin2022revisiting} & DF2K & $\checkmark$ & %
& {34.86}
& {0.9308}
& {30.76}
& {0.8505}
& {29.39}
& {0.8125}
& {29.38}
& {0.8755}
& {34.92}
& {0.9520}
\\
EDT~\cite{li2021efficient} & DF2K & $\checkmark$ & %
& 34.97
& 0.9316
& 30.89
& 0.8527
& 29.44
& 0.8142
& 29.72
& 0.8814
& 35.13
& 0.9534
\\
HAT-S~\cite{chen2023activating} & DF2K & $\checkmark$ & %
& {35.01}
& {0.9325}
& {31.05}
& {0.8550}
& {29.50}
& {0.8158}
& {30.15}
& {0.8879}
& {35.40}
& {0.9547}
\\
\hdashline
IPT~\cite{chen2021pre} & ImageNet & & $\checkmark$ %
& {34.81}
& {-}
& {30.85}
& {-}
& {29.38}
& {-}
& {29.49}
& {-}
& {-}
& {-}
\\
%EDT & ImageNet$\to$DF2K & $\checkmark$ & $\checkmark$ % & 33.06 & {0.9055} & 29.23 & {0.7971} & {27.99} & 0.7510 & 27.75 & 0.8317 & 32.39 & 0.9283 \\
%\midrule
%RCAN & DiverSeg-I (Ours) & & $\checkmark$ % & \textbf{32.70} & \textbf{0.9012} & \textbf{28.98} & \textbf{0.7908} & \textbf{27.81} & \textbf{0.7443} & \textbf{27.03} & \textbf{0.8116} & \textbf{31.58} & \textbf{0.9210}\\
\midrule
SwinIR~\cite{liang2021swinir} & DF2K & $\checkmark$ & %
& 34.97
& 0.9318
& 30.93
& 0.8534
& 29.46
& 0.8145
& 29.75
& 0.8826
& 35.12
& 0.9537
\\
SwinIR~\cite{liang2021swinir} & DiverSeg-I (Ours) &  & $\checkmark$
& \textbf{35.01}
& \textbf{0.9321}
& \textbf{31.13}
& \textbf{0.8544}
& \textbf{29.49}
& \textbf{0.8159}
& \textbf{30.12}
& \textbf{0.8869}
& \textbf{35.39}
& \textbf{0.9547}
\\
\midrule
HAT~\cite{chen2023activating} & DF2K & $\checkmark$ & %
& {35.07}
& {0.9329}
& {31.08}
& {0.8555}
& {29.54}
& {0.8167}
& {30.23}
& {0.8896}
& {35.53}
& {0.9552}
\\
HAT~\cite{chen2023activating} & ImageNet$\to$DF2K & $\checkmark$ & $\checkmark$ %
& \textbf{35.16}
& \textbf{0.9335}
& {31.33}
& {0.8576}
& {29.59}
& {0.8177}
& {30.70}
& {0.8949}
& \textbf{35.84}
& \textbf{0.9567}
\\
HAT~\cite{chen2023activating} & DiverSeg-I (Ours) & & $\checkmark$ %
& 35.14
& 0.9334
& 31.42
& \textbf{0.8577}
& \textbf{29.60}
& 0.8187
& 30.83
& 0.8965
& 35.80
& 0.9566
\\
HAT~\cite{chen2023activating} & DiverSeg-IP (Ours) & & $\checkmark$ %
& 35.10
& 0.9333
& \textbf{31.49}
& 0.8574
& \textbf{29.60}
& \textbf{0.8188}
& \textbf{30.94}
& \textbf{0.8982}
& \textbf{35.84}
& \textbf{0.9567}
\\
\bottomrule
\end{tabular}
}
%\vspace{-0.5cm}
\end{center}
\end{table}
